milliFlow: Scene Flow Estimation on mmWave Radar Point Cloud for Human Motion Sensing

Human motion sensing plays a crucial role in smart systems for decision-making, user interaction, and personalized services. Extensive research that has been conducted is predominantly based on cameras, whose intrusive nature limits their use in smart home applications. To address this, mmWave radars have gained popularity due to their privacy-friendly features. In this work, we propose milliFlow, a novel deep learning approach to estimate scene flow as complementary motion information for mmWave point cloud, serving as an intermediate level of features and directly benefiting downstream human motion sensing tasks. Experimental results demonstrate the superior performance of our method when compared with the competing approaches. Furthermore, by incorporating scene flow information, we achieve remarkable improvements in human activity recognition and human parsing and support human body part tracking. Code and dataset are available at https://github.com/Toytiny/milliFlow.

==> sections/limitation.tex <==
\vspace{-0.5em}
\section{Limitation and Future Work}
Despite the progress achieved, there are limitations to be considered in future work. First, we only experiment on a stationary radar platform where only the human subject is movable. This is akin to the scenarios of human motion sensing in smart spaces and sensors are receded into the background environment. In future work, we plan to evaluate our system on mobile platforms, such as drones and wheeled robots, where the scene flow can be induced by both ego-sensor and subject motion. Second, as a proof-of-concept work, the functioning of our method is restricted to the single subject with face-forward body motion at this stage. We plan to extend our approach to multi-person scenarios and introduce variations in the subjects' position and orientation relative to the sensor in the next study. Lastly, the number of activities included in our dataset is limited as we only design activities that can be separated into the rigid motion of multiple body skeletons. This fits our need to annotate scene flow labels based on body skeleton displacement. In our upcoming work, we will design more complex and smaller activities and exploit a novel approach to derive the scene flow.

==> sections/preliminary.tex <==
\section{SFCW mmWave radar preliminary}\label{pc_generation}
%Our objective is to estimate scene flow on point clouds generated by commercial single-chip mmWave radars. 

In this work, we employ the Vayyar radar~\cite{vayyarhome}, which is a stepped-frequency continuous-wave (SFCW) radar~\cite{weiss2009continuous} bespoken designed for fine-grained human sensing. This section aims to provide a concise overview of the point cloud generation principles of SFCW radar to aid in comprehending the hardware components of the proposed system. In what follows we introduce the working principle of SFCW radars.

\noindent\textbf{Range Estimation.}
With SFCW radar, we can detect range information with a single Tx-Rx pair. For a CW radar, the transmitting signal can be written as $s(t)=Asin(2\pi f_0 t)$, and the corresponding receiving signal from the reflection on an object at range $R$ would be $s_r(t)=A_rsin(2\pi f_0t - \phi)$, where $\phi$ is the phase difference of the transmitting and receiving signals, and can be written as $\phi = 2\pi f_0 \frac{2R}{c}$. As a result, we are able to estimate the range as $R=\frac{c}{4\pi f_0}\phi$. Note that $\phi$ can only be in range $[0, 2\pi]$. As a result, for CW radar that works on a single frequency, the maximum unambiguous range is very limited. For example, if $f_0 = 2GHz$, $R_{max} = 7.5cm$. With SFCW radar, we are able to get the phase difference at different frequencies, which provides much richer information for range estimation. For two consecutive frequencies $f_1$ and $f_2$, the frequency difference $\Delta f = f_2 - f_1$, and the phase differences at each frequency step are $\phi_1 = \frac{4\pi R}{c}f_1$ and $\phi_2 = \frac{4\pi R}{c}f_2$. We have the following equation:
\begin{equation}
% \setlength{\abovedisplayskip}{0pt}
% \setlength{\belowdisplayskip}{0pt}
    \Delta \phi = \phi_2 - \phi_1 = \frac{4 \pi R}{c}(f_2 - f_1) = \frac{4\pi R}{c} \Delta f
\end{equation}
and we get
\begin{equation}
% \setlength{\abovedisplayskip}{0pt}
% \setlength{\belowdisplayskip}{0pt}
    R=\frac{c}{4\pi \Delta f} \Delta \phi
\end{equation}
Also, we have $\Delta \phi \in [0, 2\pi]$, so the maximum unambiguous range is inversely proportional to $\Delta f$, which is the frequency step in SFCW radar. 
During each frame, the transmitter sequentially emits a series of waves of increasing frequency at equal intervals. The transmitted signal is reflected back at different surfaces in the scene and received by the receiving antenna. The ADC samples the change in amplitude and phase between the transmitted signal and the received signal and stores the values in IQ format. We can apply Fourier Transform to get the phase variation, with which we can further derive the range of the objects. This is also known as "Range-FFT". The range resolution is inversely proportional to the bandwidth of the radar, written as $R_{res} = \frac{c}{2B}$, where $B = f_{max} - f_{min}$. 

% \vspace{0.5em}
% \noindent\textbf{Clutter Removal.}
% In radar applications, each frame may contain reflections from both static and moving objects within the scene. However, when only moving targets are of interest, a sliding window approach can be employed to calculate the average response value of a sequence of frames. By subtracting this value from each frame, the response components due to the static reflections, which remain consistent across frames, are mostly eliminated. The remaining response components after subtracting the mean are then indicative of the dynamic objects present within the scene. This approach is particularly useful in our context where static background reflections are not needed for scene flow estimation.

\noindent\textbf{Angle-of-arrival Estimation.}
Angle-of-Arrival (AoA) estimation can be performed using a linear receiver array with equally-spaced elements, typically separated by a distance of $1/2 \lambda$, where the number of elements in the array, denoted as $N$, is greater than or equal to two. When a reflected signal is received at each element of the array, a phase difference arises due to the slight differences in signal travel distance, as determined by the angle of arrival, $\theta$. This phase difference can be quantified using the formula $\Delta \phi = kdsin(\theta)$, where $k$ represents the wave number and $d$ is the distance between consecutive elements. The angle of arrival can then be estimated by analyzing the phase difference using a Fourier Transform technique, commonly referred to as "Angle-FFT".
Vayyar uses Multiple-Input Multiple-Output (MIMO) array, and for each frame, we are able to get a 2D virtual antenna matrix, from which we can estimate azimuth and elevation AoA simultaneously. 

\noindent\textbf{Point Cloud Generation.}
For each frame, the raw data is stored as a complex matrix of size $N_a * N_e * M$, where $N_a$ and $N_e$ are the numbers of Tx-Rx antenna pairs (i.e., virtual antennas) in azimuth and elevation directions, respectively, and M is the number of frequency steps. First, the clutter removal is applied to focus on dynamic objects. We then apply Range-FFT for Range estimation for each virtual antenna and further perform 2D Angle-FFT to get the AoA information in both directions. Following the above processing, we are able to get a 3D heatmap for each frame.
Strong peaks are then detected with methods like CFAR~\cite{scharf1991statistical}, and converted to 3D points, which is the input to our scene flow estimation. %\chris{@Peijun, can you add CFAR somewhere in this paragraph? Kindly note that I deleted the clutter remove section for space concerns.}


% In a typical FMCW radar setting, chirp signals are emitted by the transmit (Tx) antennas in a short period of time, which are reflected by objects and then return to the receive (Rx) antennas.  Each chirp signal sweeps the frequency from low $f_{min}$ to high $f_{max}$, or vice versa and is characterized by its bandwidth $B=f_{max}-f_{min}$ and duration $T_{c}$. The intermediate frequency (IF) signal is obtained by mixing signals from a Tx-Rx pair and further sampled by the ADC to generate discrete samples for each chirp. In general, mmWave radar can produce a 3D complex data cube, aka. radar raw data, with a dimension of ${N_s\times N_c \times N_p}$ for each frame. Here, $N_s$ is the number of samples for each chirp, $N_c$ is the number of transmitted chirps in one frame and $N_p$ is the number of Tx-Rx pairs. To generate a 3D point cloud with per-point Doppler velocity, a conventional processing pipeline typically performs the following four steps based on the raw data.

% \noindent\textbf{Range-FFT.} To detect objects at different ranges, a fast Fourier transform (FFT) is first performed along the sample axis to separate different frequency components in the IF signals. Thanks to the unique sweep pattern of a chirp, the distance to the reflection objective $d$ has a linear relationship with the frequency of the IF signal $f_{IF}$ as $d = \frac{T_{c}c}{2B}f_{IF}$, where $c$ is the speed of light. Therefore, the result of the range-FFT can be seen as a "range profile" that represents the frequency responses for different ranges.  The range resolution $\Delta d$ only depends on the chirp bandwidth $B$ as $\Delta d = \frac{c}{2B}$. 

% \noindent\textbf{Doppler-FFT.} To measure the Doppler velocity, some FMCW radars transmit multiple consecutive chirps for each frame. The movement of objects can create a slight round-trip distance change between these chirps, which further yields the phase variances for the frequency peaks in the "range profile".  Another FFT can be operated along the chirp axis to extract such phase variances and the relative radial velocity $v$, aka. Doppler velocity, can be further derived as $v=\frac{\lambda}{4\pi T_{c}}\Delta\phi$,
% %As the duration $T_c$ is very short, the range of a moving object only slightly changes between chirps. Thus, the "range profile" of each chirp will still represent the responses for the identical ranges. However, the phase variance $\Delta \phi$ of certain ranges is obvious between two chirps, which can be extracted by another FFT operation along the chirp axis. 
% where $\lambda$ is the average wavelength of the chirp. The velocity resolution $\Delta v$ is determined by the chirp duration $T_c$ and the number of chirps $N_c$ as $\Delta v = \frac{\lambda}{2N_{c}T_{c}}$. After the aforementioned two FFT, the range-Doppler matrix can be generated by conducting max-pooling across the antenna axis. 

% \noindent\textbf{AoA Processing.} To calculate the exact 3D positions of objects, it is necessary to obtain their Angles of Arrival (AoA), i.e., azimuth and elevation angles. This is possible when a MIMO antenna array 
% %($N_T$ Tx antennas and $N_R$ Rx antennas) 
% is used, which has $N_p$ virtual Tx-Rx antenna pairs spatially distributed. The different distances between the objects and antenna pairs introduce phase differences between consecutive pairs. Therefore, a third and fourth FFT can be applied across the virtual azimuth and elevation dimensions to extract the AoA information of the objects. The resolution of AoA estimation depends on the number of virtual antennas pairs, the distance between antennas pairs and also the angle of the measured objects. After four FFT operated on the data cube, a 4D radar heatmap can be generated with its four axes corresponding to range, doppler velocity, azimuth and elevation. 

% \noindent\textbf{Target Detection.} To detect salient target returns against the background, a target detector like CFAR~\cite{scharf1991statistical} is usually utilized by many commercial single-chip mmWave radars after generating the heatmap. As an adaptive detection algorithm, CFAR is used to adjust the detection threshold according to the surroundings and detect outstanding peaks from the range-Doppler matrix.  The 3D positions, doppler velocity and intensities of these peaks can then be calculated with the radar heatmap and are returned as a radar point cloud in the Cartesian coordinate system.

% To summarize, given the 3D data cube, mmWave radar conducts the range-FFT, Doppler-FFT and two "Angle-FFT" to obtain a 4D radar heatmap. Strong peaks are then detected to generate a radar point cloud, which is the input to our scene flow estimation model. 


 
%as accurate Doppler velocity could significantly help our task.
%which is an advanced commercial imaging radar providing accurate 3D positional measurements of targets. Unluckily,
%with 1.6 GHz bandwidth and 40 Tx/Rx transceivers to produce high-resolution 3D radar data. 
% This radar system only transmits one chirp for each frame, thus not providing the Doppler velocity information.


% \subsection{Deep Learning Layers for Point Cloud}

% \subsubsection{Set Abstraction Layer}\label{sa_layer}
% In our radar scene flow network, we adopt the set abstraction layer proposed in PointNet++~\cite{qi2017pointnet++} as the basic learning layer to extract local point features. As an extension of PointNet~\cite{qi2017pointnet}, PointNet++~\cite{qi2017pointnet++} proposes a hierarchical structure composed of multiple set abstraction levels. At each level, the local features of a set of points are abstracted and taken as the input to the next level. The working process of each set abstraction layer can be summarized in three steps. First, the iterative farthest point sampling (FPS) is applied to select $N'$ points the point sets as the centroids for local regions. Second, the ball query identifies neighbour points within a radius $R$ of each centroid, resulting in $N'$ local point sets.  Lastly, the local region features are encoded for each centroid using the PointNet layer~\cite{qi2017pointnet}, which is composed of an MLP to extract high-level representations and a max-pooling layer to aggregate the representations of all local points to the centroid. The output is the per-point local features for $N'$ selected points at a specific scale determined by the radius $R$. 

% \subsubsection{Cost Volume Layer}\label{cv_layer}
% To encode points motion between two radar frames, in our network design, we leverage the point cloud cost volume layer in~\cite{wu2020pointpwc} to correlate features. In the cost volume layer, the matching costs $Cost(p_i, q_j)$ of all point pairs $(p_i, q_j)$ between two point clouds $\mathcal{P}$ and $\mathcal{Q}$ are first calculated through an MLP. Then, the costs are aggregated in a patch-to-patch manner to produce robust and stable cost volumes. During aggregation, the neighbourhood is first found for each point $p_c$ in $\mathcal{P}$. Then, for each neighbour point $p_i$ of $p_c$, a neighbourhood is found around it in $\mathcal{Q}$. With these patches in $\mathcal{Q}$ and $\mathcal{P}$, the costs can be aggregated respectively through a weight-sum operation whose weights are leanrable parameters from MLPs. The output is two-dimension cost volumes with shape $N\times D$, where $N$ is the number of points of the point cloud $\mathcal{P}$ and $D$ is the dimension of the cost volume.
